Output Feedback Minimax Adaptive Control

This paper formulates adaptive controller design as a minimax dual control problem. The objective is to design a controller that minimizes the worst-case performance over a set of uncertain systems. The uncertainty is described by a set of linear time-invariant systems with unknown parameters. The main contribution is a common framework for both state feedback and output feedback control. We show that for finite uncertainty sets, the minimax dual control problem admits a finite-dimensional information state. This information state can be used to design adaptive controllers that ensure that the closed-loop has finite gain. The controllers are derived from a set of Bellman inequalities that are amenable to numerical solutions. The proposed framework is illustrated on a challenging numerical example.

==> figures/src/tikzpreamble.tex <==
\usepackage{pgfplots, tikz, pgfplotstable}
\pdfminorversion=4
\usepackage{amsmath, amssymb}
\usetikzlibrary{positioning, shapes, arrows, calc}
\tikzstyle{block} = [draw, rectangle, line width=0.7mm]
\tikzstyle{sumcircle} = [draw, circle, line width=0.7mm]

\def \plotwidth {8.5cm}
\def \plotheight {4cm}

% Ensure that the plots have fonts consistent with the rest of the document

% IEEE uses Times font, so we'll default to times.
% These three commands make up the entire times.sty package.
%renewcommand{\sfdefault}{phv}
%\renewcommand{\rmdefault}{ptm}
%\renewcommand{\ttdefault}{pcr}


==> tex/preliminaries.tex <==
\subsection{Full-Information linear quadratic control}
\begin{problem}[Full-Information]\label{prob:prel:FI}
	Let  $H \in \S^{n_z + n_u + n_d}$ satisfy
	\begin{equation}\label{eq:prel:FI:H}
		\begin{aligned}
			H & = \bmat{
			H^{zz} & H^{zu} & H^{zd} \\
			H^{uz} & H^{uu} & H^{ud} \\
			H^{dz} & H^{du} & H^{dd}
		},
		& \begin{aligned}
			H^{dd} & \prec 0, \\
			H / H^{dd} & \succeq 0, \\
			[H / H^{dd}]^{uu} & \succ 0.
		\end{aligned}
	\end{aligned}
	\end{equation}
	Compute
	\begin{equation}\label{eq:prel:FI:objective}
		\inf_\mu\sup_{d, N} \sum_{t=0}^{N-1} \left |(\hat z_t, u_t, d_t) \right|^2_{H},
	\end{equation}
	where $N \geq 0$ and the sequences, $\seq{z}{0}{N},\ \seq{u}{0}{N-1}$ are generated by
	\begin{align}
		z_{t + 1} & = A z_t + B u_t + G d_t, \quad t \geq 0, \label{eq:known_dynamics:dynamics}\\
		u_t & = \mu_t(z_0, \ldots, z_t, d_0, \ldots, d_{t-1}, u_0, \ldots, u_{t-1}). \label{eq:known_dynamics:control_law}
	\end{align}
\end{problem}
For functions $V : \R^{n_z} \to \R$, we define the Bellman operators
\begin{equation}\label{eq:prel:FI:B}
	\B V(z) \defeq \min_u \underbrace{\max_d\left\{ V(Az + Bu + Gd) + |(z, u, d)|^2_H \right\}}_{\B_uV(z)},
\end{equation}
and the value iteration
\begin{subequations}\label{eq:prel:FI:value_iteration}
	\begin{align}
		V_0(z) & = 0, \\
		V_{k + 1}(z) & = \B V_k(z), \quad k \geq 0.
	\end{align}
\end{subequations}%
\newcounter{prop:prel:FI}%
\begin{prop}
	The following facts holds for Problem~\ref{prob:prel:FI}, the Bellman operator $\B$ in \eqref{eq:prel:FI:B} and the value iteration defined in \eqref{eq:prel:FI:value_iteration}.
	\begin{enumerate}
		\item $\B$ is monotone, i.e., $V' \geq V \implies \B V' \geq \B V$.
		\item The value iteration is non-decreasing;  $V_{k + 1} \geq V_k$.
		\item The value iteration converges if and only if it is bounded.
		\item The value~\eqref{eq:prel:FI:objective} is bounded if and only if the value iteration converges.
			\setcounter{prop:prel:FI}{\value{enumi}}
	\end{enumerate}

If the value iteration converges to a limit $V_\star$, then
	\begin{enumerate}
		\setcounter{enumi}{\value{prop:prel:FI}}
		\item The value \eqref{eq:prel:FI:objective} is equal to $V_\star(z_0)$.
		\item $V_\star$ is a fixed point of $\B$, not necessarily unique.
		\item $V_\star$ is the minimal non-negative fixed point of $\B$. I.e., for all other non-negative fixed points $\bar V$, $V_\star(z) \leq \bar V(z)$ for all $z \in \R^{n_x}$, and for some $\bar z \in \R^{n_z}$, $V_\star(\bar z) < \bar V(\bar z)$.
	\end{enumerate}
\end{prop}


\subsection{Output-feedback linear quadratic control}
We now consider the problem of output-feedback linear quadratic control and show to to reduce it to an instance of the full-information problem.
\begin{problem}[Output-feedback minimax control]\label{prob:prel:output_feedback}
	Let $Q \in \S^{n_x}$, $R \in \S^{n_u}$, be positive definite. 
	Given a model $(A, B, G, C, D) \in \R^{n_x \times n_x} \times \R^{n_x \times n_u} \times \R^{n_x \times n_w} \times \R^{n_y \times n_x} \times \R^{n_y \times n_v}$ and a positive quantity $\gamma > 0$ , compute
	\begin{equation}\label{eq:prel:output_feedback:objective}
		\inf_\mu\sup_{w, v,  N} \sum_{t=0}^{N-1} \left(|x_t|^2_Q + |u_t|^2_R - \gamma^2|(w_t, v_t)|^2 \right) - |x_0 - \hat x_ 0|^2_{S_0},
	\end{equation}
	where $w_t \in \R^{n_w}$, $v_t \in \R^{n_v}$ $N \geq 0$, and the sequences, $\seq{x}{0}{N}$, $\seq{y}{0}{N-1}$ and $\seq{u}{0}{N-1}$ are generated by
\begin{subequations}\label{eq:prel:output_feedback:system}
	\begin{align}
		x_{t + 1} & = A x_t + B u_t + Gw_t, \quad t \geq 0 \label{eq:prel:output_feedback:dynamics}\\
		y_t & = C x_t + D v_t, \label{eq:prel:output_feedback:output}\\
		u_t & = \mu_t(y_0, \ldots, y_{t-1}, u_0, \ldots, u_{t-1}). \label{eq:prel:output_feedback:control_law}
	\end{align}
\end{subequations}
\end{problem}

We make the following assumptions
\begin{assumption}[Problem parameters]\label{assumption:prel:output_feedback:problem}
	The matrices 
	$\bmat{
			A & G \\ 
		}
	$
	and $D$ are surjective, $\bmat{A^\tran & \sqrt{Q}}^\tran$ is injective
\end{assumption}
Define 
\begin{multline}\label{eq:prel:output_feedback:W}
	W^{N}(x, \seq{u}{0}{N-1}, \seq{y}{0}{N-1}) = 	\sup_{\seq{w}{0}{N-1}, \seq{v}{0}{N-1}} \Big\{ - |x_0 - \hat x_0|^2_{S_0^{-1}} \\
 + \sum_{t=0}^{N-1} \left(|x_t|^2_Q + |u_t|^2_R - \gamma^2|(w_t, v_t)|^2\right)  \Big \},
\end{multline}
where the supremum is taken subject to the dynamics \eqref{eq:prel:output_feedback:dynamics} and \eqref{eq:prel:output_feedback:output} having generated the sequences $\seq{y}{0}{N-1}$, and $\seq{u}{0}{N-1}$, with $x_N = x$. 
The value \eqref{eq:prel:output_feedback:objective} is then equal to
\[
	\inf_\mu \sup_{N, \seq{y}{0}{N-1}, x} W^N(x, \seq{u}{0}{N-1}, \seq{y}{0}{N-1}).
\]

This reformulation has two major benefits. 
The first is that minimizing over $\mu_t$ and maximizing over $\seq{y}{0}{t-1}$ commutes as $\mu_t$ is a function of $\seq{y}{0}{t-1}$.
This interchange of extremization leads to a sequantial optimization problem that can be solved by dynamic programming.
The second benefit is that $W^N$ can be computed recursively in a manner that reduces the output-feedback problem to the principal problem.

The following lemma summarizes the recursive computation of $W^N$, we refer the reader to~\cite[Chapter 6]{Basar95} for a proof.
The expression of $r_{t+1}$ is unnecessary when one employs the certainty equivalence principle of~\cite{Basar95}, but is crucial to our theory of adaptive control.

\begin{lemma}\label{lemma:prel:output_feedback:W}
		With matrices $A$, $B$, $G$, $C$, $D$, $Q$, $R$, $S_0$, and $\hat x_0$ as in Problem~\ref{prob:prel:output_feedback}, let $S_{t + 1} \in \S^{n_x}$, $X_t \in \S^{n_y}$, and $L_t \in \R^{n_x \times n_y}$ be defined recursively for $t = 0, 1, \ldots$ by
	\begin{subequations}\label{eq:prel:output_feedback:forward_riccati}
	\begin{align}
		S_{t+1} & = (A X_t^{-1} A^\tran + \gamma^{-2}GG^\tran)^{-1}, \\
		X_t & = S_t + \gamma^2 C^\tran(DD^\tran)^{-1} C - Q, \\
		L_t & = \gamma^2 A X_t^{-1} C^\tran(DD^\tran)^{-1}.
	\end{align}
	If $S_t\succ Q$ for all $t = 0, \ldots, N$, then $W^N$ defined by \eqref{eq:prel:output_feedback:W} satisfies
	\begin{equation}\label{eq:prel:output_feedback:W^N}
	W^N(x, \seq{u}{0}{N-1}, \seq{y}{0}{N-1}) = -|x - \hat x_N|^2_{S_N} + r_N,
	\end{equation}
\end{subequations}
	where $r_0 = 0$ and
	\begin{subequations}\label{eq:prel:prel:output_feedback:observers}
	\begin{align}
		&\hat x_{t + 1} = A \hat x_{t} + Bu_t + L_t(y_t - C \hat x_{t}) +AX_t^{-1}Q\hat x_t, \\
		&\, r_{t + 1}  = r_t + |\hat x_{ t}|^2_{(Q^{-1} - S_t^{-1})^{-1}} + |u_t|^2_R \\
			  & \quad - |y_t - C (S - Q)^{-1}S\hat x_{ t}|^2_{(DD^\tran / \gamma^2 + C(S - Q)^{-1}C^\tran)^{-1}}.
	\end{align}
\end{subequations}
If, for any $t \geq 0$, $S_t^{-1} \nsucceq Q$, then the value \eqref{eq:prel:output_feedback:objective} is unbounded.
\end{lemma}

\begin{remark}
	Note that
	\[
		r_{t} = \sum_{\tau = 0}^{t-1} |(\hat x_{\tau}, u_\tau, y_\tau)|^2_{\hat Q_{\tau}},
	\]
	where
	\begin{equation}\label{eq:prel:output_feedback:Q_tau}
		\begin{aligned}
		 & 	\hat Q^{xx}_{\tau} =  S_\tau X_\tau^{-1} S_\tau - S_\tau, \quad \hat Q^{xu}_{\tau} = 0, \\
		 &	\hat Q^{uu}_{\tau} = R, \quad
		 	\quad \hat Q^{yy}_{\tau} = -(DD^\tran / \gamma^2 + C(S_\tau - Q)^{-1})^{-1}, \\
		 &	\hat Q^{uy}_{\tau} = 0, \quad
		 \hat Q^{xy}_{\tau} = \gamma^2 S_\tau X_\tau^{-1}C^\tran(DD^\tran)^{-1}.
		\end{aligned}
	\end{equation}
\end{remark}


\begin{theorem}[Reduction]\label{thm:prel:output_feedback:reduction}
	For Problem~\ref{prob:prel:output_feedback}, under Assumption~\ref{assumption:output_feedback:problem}, the following statements are true:
	\begin{enumerate}
		\item There exists a finite $\gamma > 0$ so that the sequences~\eqref{eq:prel:output_feedback:forward_riccati} converge to limits $S$ and $X$ that are positive definite matrices and $AX^{-1}S$ is Schur stable.
		\item Given $\gamma > 0$, the value~\eqref{eq:prel:output_feedback:objective} is bounded only if the sequences~\eqref{eq:prel:output_feedback:forward_riccati} converge to a solution such that $S \succ Q$.
		\item If the condition in statement 2) holds, let $\hat A = AX^{-1}S$, $\hat B = B$, $\hat G = L$, and let $\hat Q$ be the corresponding limit of~\eqref{eq:prel:output_feedback:Q_tau}.
			If $S_0 = S$, then the value \eqref{eq:prel:output_feedback:objective} is equal to
			\begin{equation}\label{eq:prel:output_feedback:reduced}
				\inf_{\hat \mu}\sup_{y, N}\sum_{t=0}^{N-1}|(\hat x_t, u_t, y_t)|^2_{\hat Q},
			\end{equation}
				where the sequences $\hat x_t$ and $u_t$ are generated by
			\[
				\begin{aligned}
					\hat x_{t+1} & = \hat A x_t + \hat B u_t + \hat G y_t, \\
					u_t & = \hat \mu_t(\hat x_0, \ldots, \hat x_t, u_0, \ldots, u_{t-1}, y_0, \ldots, y_{t-1}).
				\end{aligned}
			\]
			A controller $\hat \mu^\star$ is optimal for~\eqref{eq:prel:output_feedback:reduced} if and only if it is optimal Problem~\ref{prob:prel:output_feedback}.
	\end{enumerate}

\end{theorem}

	\onote{
	\begin{enumerate}
		\item Jag är inte helt 100 på bevisföringen här. Får läsa på, är egentligen inte ett helt nödvändigt påstående, men vore fint att kunna säga detta. Eventuellt måste man också kunna skala $S_0$.
		\item Jag förstår faktiskt inte konvergensegenskaperna hos sekvensen helt, men kravet på att $S_t \succ Q$ är nödvändigt för att kostnaden ska vara begränsad. Det är antagligen så att $\lim_{t \to \infty} S_t$ beror på $S_0$, alltså att Riccati kan ha flera lösningar.
		\item Detta är själva reduceringen som vi är intresserade av. De två översta punkterna är bara för att motivera varför vi alltid kan välja ett gamma så att omskrivningen existerar.
	\end{enumerate}
	}
	\begin{proof}[Proof statement 3]
		From Lemma~\ref{lemma:prel:output_feedback:W}, we know that for a fixed policy $\mu$ and horizon $N \geq 0$, the value of the inner optimization problem in~\eqref{eq:prel:output_feedback:objective},
\begin{multline*}
	\sup_{w, v} \left\{\sum_{t = 0}^{N-1}\left(|x_t|^2_Q + |u_t|^2_R - \gamma^2|(w_t, v_t)|^2\right) - |x_0 - \hat x_0|^2_{S_0} \right\} \\
	=
	\sup_{\seq{y}{0}{N-1}, x}\left\{
	-|x - \hat x_N|_{S_N} + \sum_{\tau = 0}^{N - 1}|(\hat x_{\tau}, u_\tau, y_\tau)|^2_{\hat Q_{\tau}}
	\right\} \defeq J_N^\mu(\hat x_0),
\end{multline*}
	where $\hat Q_{\tau}$ is defined in~\eqref{eq:prel:output_feedback:Q_tau} and the sequences $\hat x_t$ and $u_t$ are generated by~\eqref{eq:prel:output_feedback:observers}.
	As $S_N$ is positive definite, the unique maximizing argument is $x_\star = \hat x_N$.
	By assumption, $S_0$ is a stationary solution to the Riccati equation~\eqref{eq:prel:output_feedback:forward_riccati} and therefore $S_t = S = S_0$ and the corresponding matrices $\hat Q_t$, $X_t$, $L_t$, $\hat A$, $\hat B$ and $\hat G$ are also stationary.
	Finally, as $\hat x_t$ is a function of $\seq{y}{0}{t-1}$ and $\seq{u}{0}{t-1}$, the sets of feasible controllers $\mu$ in Problem~\ref{prob:prel:output_feedback} and $\hat \mu$ in this theorem are equal.
	We conclude that the optimal values are equal.
\end{proof}


==> tex/probform.tex <==



